DynaMiTe: A Dynamic Local Motion Model with Temporal Constraints for Robust Real-Time Feature Matching

Feature based visual odometry and SLAM methods require accurate and fast correspondence matching between consecutive image frames for precise camera pose estimation in real-time. Current feature matching pipelines either rely solely on the descriptive capabilities of the feature extractor or need computationally complex optimization schemes. We present the lightweight pipeline DynaMiTe, which is agnostic to the descriptor input and leverages spatial-temporal cues with efficient statistical measures. The theoretical backbone of the method lies within a probabilistic formulation of feature matching and the respective study of physically motivated constraints. A dynamically adaptable local motion model encapsulates groups of features in an efficient data structure. Temporal constraints transfer information of the local motion model across time, thus additionally reducing the search space complexity for matching. DynaMiTe achieves superior results both in terms of matching accuracy and camera pose estimation with high frame rates, outperforming state-of-the-art matching methods while being computationally more efficient.

==> sections/conclusion.tex <==
\section{Conclusion}\noindent
The superior results of \textit{DynaMiTe} and the high framerate capabilities that only require CPU usage for robust feature matching from consecutive image frames indicate possible applications in visual odometry or SLAM. Due to its efficient implementation many SLAM scenarios for handheld devices, AR/VR or UAVs are possible use cases for the proposed method.
As the joint formulation of \textit{DynaMiTe}, with its \textit{spatial} and \textit{temporal} constraints, can be better expressed in consecutive image frames, a video of \textit{DynaMiTe} can be found in the supplementary material.\footnote{The size restriction of the supplementary material only allowed for a low-quality rendering. In accordance with the review process a high-quality video will be linked with the camera-ready version of the paper.}

==> sections/experiments.tex <==
\section{Experiments}
\label{Experiments}\noindent
%Pose error evaluation is performed on the TUM-RGBD~\cite{sturm2012benchmark} benchmark with the same split as~\cite{bian2017gms}. We use one Kitti sequence (odometry sequence 00)~\cite{geiger2013vision}, and the static webcam dataset from~\cite{TILDE} for reprojection accuracy evaluations.

%We use the following datasets:
%\begin{enumerate}
%\item TUM~\cite{sturm2012benchmark}
%\item Kitti~\cite{geiger2013vision}~\cite{sturm2012benchmark}
%\item Carla~\cite{Dosovitskiy17}
%\item Webcam~\cite{TILDE}
%\end{enumerate}

We perform following experiments for evaluation:
\begin{enumerate}
\item Accuracy:
%For the feature match accuracy, we compute the fundamental matrix \(F\) from ground truth camera poses and calculate the distance between points of correspondences and their respective epipolar lines~\cite{Hartley:2000:MVG:375372}:
%\begin{equation}
%d\left(p,Fp_{\prime}\right) = \frac{p^{\prime T}Fp}{\sqrt{\left(Fp\right)_{\left[1\right]}^{2} + \left(Fp\right)_{\left[2\right]}^{2}}},
%\end{equation}
%where \(p=\left[u,v,1\right]^T\) and \(p^{\prime}=\left[u^{\prime},v^{\prime},1\right]^T\) are homogeneous coordinates of the feature matches. We report the symmetric epipolar distance~\cite{yi2018learning} \(E_{d}=d\left(p,Fp_{\prime}\right) + d\left(p^{\prime},E^{T}p_{\prime}\right)\) as one accuracy measure.
%The TUM-RGBD~\cite{sturm2012benchmark} benchmark with the same split as~\cite{bian2017gms} is used

\end{enumerate}



%Structure:
%\begin{enumerate}
%\item Quantitative Evaluation on matching accuracy with rendered MPI Sintel dataset \cite{Butler:ECCV:2012} with ground truth for depth. We take the ground truth camera poses of the stereo set and triangulate the matched sparse feature points between the left and right view and compare the computed depth value with the corresponding pixel location in the disparity ground truth for validation. We analyze the precision, recall and F-measure for different matching methods.
%\item Quantitative analysis of runtime in relation to number of feature points
%\item Quantitative evaluation on pose estimation from different visual odometry datasets with pose ground truth: we analyze the pose estimation from frame to frame and also consider accumulated drift over time; we compare different matching algorithms and take the output matches for simple pose computation disregarding scale; further we also compare to fully developed visual odometry methods methods and SLAM pipelines with bundle adjustment, optimization techniques and loop closures
%\end{enumerate}

%Experiments and evaluation.
%\begin{figure}[htbp]
%\includegraphics[width=0.47\textwidth]{graphics/runtime2.png}
%\caption{Runtime analysis for DLMM}
%\label{Evaluation_Runtime_1}
%\end{figure}

%\paragraph{VIO Datasets}
%KITTI odometry~\cite{geiger2013vision}
%Malaga urban~\cite{blanco2014malaga}
%UMich NCLT~\cite{carlevaris2016university}
%The EuRoC MAV dataset includes 11 outdoor sequences~\cite{burri2016euroc}
%PennCOSYVIO~\cite{pfrommer2017penncosyvio}
%Zurich Urban MAV~\cite{tillzurich}
%TUM VI~\cite{schubert2018vidataset}

%HPatches: https://github.com/hpatches/hpatches-dataset

%\todo{evaluation on pose}\\
%\todo{evaluation on slam}\\


%\todo{evaluation on different datasets and on real data}\\
%\todo{https://jwbian.net/matchbench}\\
%\todo{https://github.com/MagicLeapResearch/SuperPointPretrainedNetwork/blob/master/assets/DL4VSLAM_talk.pdf}


%\todo{Comments and Feedback from Kick-Off:\\
%- use unrectified images\\
%- use images from different cameras/sensors and show applicability for matching between %those\\
%- dynamic patch size (e.g. based on priors or region growing)}\\

